Jefferson Lab Hall C: Precision Physics at the Luminosity Frontier

Over the last three decades, Hall C has been a key contributor to progress in the understanding of hadron structure and interactions. An outline of a potential future Hall C physics program focused on precision measurements of small cross sections is presented. A detailed overview of this unique facility, whose flexible configuration allows many opportunities for new experimental equipment that help address a wide range of questions in hadronic physics, is included as well.

==> CPS_e+e-/CPS_e+e-references.tex <==
\begin{thebibliography}{0}
%
\bibitem{MJ2000} M. K. Jones et al., Phys. Rev. Lett. 84, 1398 (2000); V. Punjabi et al., Phys. Rev. C 71, 055202 (2005); 71, 069902(E) (2005).
%
\bibitem{EC2021} E. M. Christy et al., arXiv:2103.01842.
%
\bibitem{SLAC} J. Mar et al., Phys. Rev. Lett. 21, 482 (1968).
%
\bibitem{IR2015} I. A. Rachek et al., Phys. Rev. Lett. 114, 062005 (2015).
%
\bibitem{BH2017} B. S. Henderson et al., PRL 118, 092501 (2017).
%
\bibitem{DR2017} D. Rimal et al., Phys. Rev. C 95, 065201 (2017).
%
\bibitem{OL2019} D. Hasell et al., A Future Two-photon Exchange Experiment at DESY, APS April Meeting 2019.
%
\bibitem{DD2020} D. Day et al., NIM A, 957, 163429 (2020).
%
\bibitem{BW2017} B. Wojtsekhowski and G. Niculescu, arXiv:1712.06419.
%
\bibitem{BW2009} B. Wojtsekhowski, AIP Conf. Proc. 1160, 149 (2009), arXiv:0906.5265. 
%
\bibitem{PADME} M. Raggi, V. Kozhuharov, Advances in High Energy Physics, vol. 2014, ID 959802 (2014).
%
\end{thebibliography}

==> HMS_upgrade.tex <==
A Hall C Upgrade after a CEBAF Upgrade to 22 GeV/c
Would hall C have a feasible upgrade path assuming that the CEBAF is upgraded to 22 GeV/c ? The answer to this question requires a quick examination of the two spectrometers, HMS and SHMS and their current features. SHMS was designed to replace SOS and keep Hall C’s capability to always have a beam energy electron spectrometer. Execution of SHMS in the space left behind after the SOS was removed required using magnets with peak fields of 5 Tesla and squeezing the design to make best use of the space available. Indeed, the end of the dipole is just inside the Detector shield house. HMS on the other hand was built to be very conservative and used 2 Tesla magnets, long effective field lengths and a lot of drift space. Even with this conservatism HMS was designed to ultimately reach 6 GeV/c and still not have magnets at full current. The HMS dipole bend limit is 7.5 Gev/c while the focusing limit is about 7.2 Gev/c. Just as an aside, the HMS quads were even more conservative in that Oxford built in an extra 20\% into the quads, power supplies and current leads as they had doubt about how the saturated iron would perform. Upgrading SHMS would require use of 10 Tesla magnets. Small bore 10 Tesla magnets for LHC upgrades have been built but stretching this technology to large bore large acceptance spectrometer magnets is another story. The HMS on the other hand uses 2 Tesla magnets to reach over 7 Gev/c would require about 6 Tesla magnets to reach 22 Gev/c. Magnets that can reach 6 Tesla can be built today using NbTi superconductors running at 4.2 kelvin. Careful magnet design that squeezes the drift space out of the HMS and increases the magnets effective lengths would lower the maximum field requirement even lower. The dipole would likely have to be split into two or “bent” in order to have a large acceptance at a 30 degree bend. Two dipole is a common cryostat with a “kink” would be the easiest path to 22 GeV/c. Similarly the three quads could be mounted in a common cryostat which would permit longer effective lengths. A clone of the SHMS HB would be required to reach very small angles. The HMS has a clear, reasonable, feasible and affordable path to 22 GeV/c.
Upgrading HMS would involve removing the present magnets and overhead steel structure, procuring a new suite of magnets and installation. This project would be comparable in effort and cost to the SHMS project and thus would require 8-9 years and 25-30 millions of dollars. The entire HMS pivot assembly, support structure and shield house would be reused as is. Magnet engineering would take ~ 2 years, magnet procurement would take 1 year and magnet contract execution 4 years. HMS disassembly would require about 1 year and could be started just prior to the arrival of the first 22 GeV/c new magnets. HMS- Super (HMS$^2$) installation would take about one year and one year should be allowed for commissioning. The existing HMS cryo distribution line and magnet u-tubes could be re-used and possibly the magnet controls could be re-used. New DC power supplies are likely required. Small items like the HMS vacuum connector pieces would have to be examined for reuse.
JLAB has the manpower available in house for this project.


%
To match the accelerator energy of 22~GeV, the HMS can be upgraded to 
accept particles with momentum of  22~GeV/c and reach small scattering angles.
The present HMS was built conservatively to reach 7.2~GeV/c by using 2 Tesla magnets with long effective field lengths 
and plenty of drift space. To reach 22~GeV/c, the HMS magnets would need to operate at 6 Tesla which 
can be achieved with present day superconducting magnets. As with the SHMS, a horizontal bending magnet would be needed to allow the HMS to access small scattering angles. Upgrading HMS would involve removing the present magnets and overhead steel structure, procuring a new suite of magnets and installation. The entire HMS pivot assembly, support structure and shield house could be reused. For the experiments presented in this paper, the present HMS momentum range is sufficient. 
We encourage physics proposals that would need an expanded HMS momentum range and would define the HMS upgrade. 






==> Makefile <==
# absolutely trivial makefile that makes SHMS NIM article pdf
# H. Fenker
#
DocName=main
REV=NONE

pdf: */*.tex
	pdflatex $(DocName).tex
	bibtex $(DocName)
	pdflatex $(DocName).tex
	pdflatex $(DocName).tex
	@echo -e '\n\n                 ---------- WARNINGS ----------\n\n'
	grep Warning $(DocName).log | grep -v 'float specifier changed'
	@echo -e '\n\n                 ------------------------------\n\n'

diff:
ifeq ($(REV),NONE)
	@echo ''
	@echo 'Usage:  make REV=<git sha1>'
	@echo '    Use 'git log' and choose the commit you want to compare to.'
	@echo '    A new PDF will be generated with removals/addtions in red/blue.'
	@echo ''
else
	latexdiff-git --force --flatten --pdf -r $(REV) $(DocName).tex
endif

clean:
	rm -f $(DocName).{out,log,spl,bbl,blg,brf} *.aux ${DocName}Notes.bib

